Probabilistic Planning with Preferences over Temporal Goals

We present a formal language for specifying qualitative preferences over temporal goals and a preference-based planning method in stochastic systems. Using automata-theoretic modeling, the proposed specification allows us to express preferences over different sets of outcomes, where each outcome describes a set of temporal sequences of subgoals. We define the value of preference satisfaction given a stochastic process over possible outcomes and develop an algorithm for time-constrained probabilistic planning in labeled Markov decision processes where an agent aims to maximally satisfy its preference formula within a pre-defined finite time duration. We present experimental results using a stochastic gridworld example and discuss possible extensions of the proposed preference model.

==> chain_mdp.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3.5cm,
        scale = 0.5,transform shape]
  \node[state] (0) [initial] {$0$};
  \node[state] (1) [right of=0] {$1$};
  \node[state] (2) [right of=1] {$2$};
  \node[state] (3) [right of=2] {$3$};
  \node[state] (4) [right of=3] {$4$};
  \node[state] (5) [right of=4] {$5$};
  \node[state] (6) [right of=5] {$6$};
  \node[state] (7) [right of=6] {$7$};
  \node[state] (8) [below of=3] {$8$};

  \path (0) edge              node {$a:0.8$} (1)
        (0) edge   [loop above]           node {$a:0.1$} (0)
        (0) edge              node {$a:0.1$} (8)
        (1) edge              node {$a:0.8$} (2)
        (1) edge   [loop above]           node {$a:0.1$} (1)
        (1) edge              node {$a:0.1$} (8)
        (2) edge              node {$a:0.8$} (3)
        (2) edge    [loop above]          node {$a:0.1$} (2)
        (2) edge              node {$a:0.1$} (8)
        (3) edge              node {$a:0.8$} (4)
        (3) edge    [loop above]          node {$a:0.1$} (3)
        (3) edge              node {$a:0.1$} (8)
        (4) edge              node {$a:0.8$} (5)
        (4) edge    [loop above]          node {$a:0.1$} (4)
        (4) edge              node {$a:0.1$} (8)
        (5) edge              node {$a:0.8$} (6)
        (5) edge    [loop above]          node {$a:0.1$} (5)
        (5) edge              node {$a:0.1$} (8) 
        (6) edge              node {$a:0.8$} (7)
        (6) edge    [loop above]          node {$a:0.1$} (6)
        (6) edge              node {$a:0.1$} (8)       
        (7) edge    [loop above]          node {$a:1$} (7)
        (8) edge    [loop left]          node {$a:1$} (8);
\end{tikzpicture}
